Multipath-based Localization and Tracking considering Off-Body Channel Effects

This paper deals with multipath-based positioning and tracking in off-body channels. An analysis of the effects introduced by the human body and the implications on positioning and tracking is presented based on channel measurements obtained in an indoor scenario. It shows the influence of the radio signal bandwidth on the human body induced field of view (FOV) and the number of multipath components (MPCs) detected and estimated by a deterministic maximum likelihood (ML) algorithm. A multipath-based positioning and tracking algorithm is proposed that associates these estimated MPC parameters with floor plan features and exploits a human body-dependent FOV function. The proposed algorithm is able to provide accurate position estimates even for an off-body radio channel in a multipath-prone environment with the signal bandwidth found to be a limiting factor.

==> figures/m120_K_CDF/m120_K_CDF.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.9\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=20,
%xlabel style={font=\color{white!15!black}},
xlabel={number of estimated SMCs $\hat{K}^{(j)}$},
ymin=0,
ymax=1,
%ylabel style={font=\color{white!15!black}},
ylabel={CDF},
%axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(1.01,1)}, anchor=north west, legend cell align=left, align=left, draw=black,fill=white},
%extraAxisOptions,
% unit vector ratio=1 1 1
grid style=dotted,
major tick length=1mm,
clip mode=individual,
xlabel style = {yshift=1.5mm},
ylabel style = {yshift=-1mm},
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BW= 4GHZ
\addplot [color=red, dashed, line width=0.75pt,forget plot]
  table[]{\datapath/m120_fc6950MHz_bw3939MHz_K_CDF-1.tsv};
% \addlegendentry{$\hat{K}^{(1)}$}%{total (A1)}

\addplot [color=red, line width=0.75pt]
  table[]{\datapath/m120_fc6950MHz_bw3939MHz_K_CDF-2.tsv};
\addlegendentry{$\vm{a}^{(1)}$}%{$\hat{K}_{\mathrm{OSPA}}^{(1)}$}%{associated (A1)}

\addplot [color=blue, dashed, line width=0.75pt,forget plot]
  table[]{\datapath/m120_fc6950MHz_bw3939MHz_K_CDF-3.tsv};
% \addlegendentry{$\hat{K}^{(2)}$}%{total (A2)}

\addplot [color=blue, line width=0.75pt]
  table[]{\datapath/m120_fc6950MHz_bw3939MHz_K_CDF-4.tsv};
\addlegendentry{$\vm{a}^{(2)}$}%{$\hat{K}_{\mathrm{OSPA}}^{(2)}$}%{associated (A2)}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BW= 2GHZ
\addplot [color=red, dashed, line width=0.75pt,forget plot]
  table[]{\datapath/m120_fc6950MHz_bw2000MHz_K_CDF-1.tsv};
% \addlegendentry{$\hat{K}^{(1)}$}%{total (A1)}

\addplot [color=red, line width=0.75pt]
  table[]{\datapath/m120_fc6950MHz_bw2000MHz_K_CDF-2.tsv};
\addlegendentry{$\vm{a}^{(1)}$}%{$\hat{K}_{\mathrm{OSPA}}^{(1)}$}%{associated (A1)}

\addplot [color=blue, dashed, line width=0.75pt,forget plot]
  table[]{\datapath/m120_fc6950MHz_bw2000MHz_K_CDF-3.tsv};
% \addlegendentry{$\hat{K}^{(2)}$}%{total (A2)}

\addplot [color=blue, line width=0.75pt]
  table[]{\datapath/m120_fc6950MHz_bw2000MHz_K_CDF-4.tsv};
\addlegendentry{$\vm{a}^{(2)}$}%{$\hat{K}_{\mathrm{OSPA}}^{(2)}$}%{associated (A2)}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % BW= 1GHZ
% \addplot [color=red, dashed, line width=0.75pt,forget plot]
%   table[]{\datapath/m120_fc6950MHz_bw1000MHz_K_CDF-1.tsv};
% % \addlegendentry{$\hat{K}^{(1)}$}%{total (A1)}
% 
% \addplot [color=red, line width=0.75pt]
%   table[]{\datapath/m120_fc6950MHz_bw1000MHz_K_CDF-2.tsv};
% \addlegendentry{$\vm{a}^{(1)}$}%{$\hat{K}_{\mathrm{OSPA}}^{(1)}$}%{associated (A1)}
% 
% \addplot [color=blue, dashed, line width=0.75pt,forget plot]
%   table[]{\datapath/m120_fc6950MHz_bw1000MHz_K_CDF-3.tsv};
% % \addlegendentry{$\hat{K}^{(2)}$}%{total (A2)}
% 
% \addplot [color=blue, line width=0.75pt]
%   table[]{\datapath/m120_fc6950MHz_bw1000MHz_K_CDF-4.tsv};
% \addlegendentry{$\vm{a}^{(2)}$}%{$\hat{K}_{\mathrm{OSPA}}^{(2)}$}%{associated (A2)}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BW= 500MHZ
\addplot [color=red, dashed, line width=0.75pt,forget plot]
  table[]{\datapath/m120_fc6950MHz_bw0500MHz_K_CDF-1.tsv};
% \addlegendentry{$\hat{K}^{(1)}$}%{total (A1)}

\addplot [color=red, line width=0.75pt]
  table[]{\datapath/m120_fc6950MHz_bw0500MHz_K_CDF-2.tsv};
\addlegendentry{$\vm{a}^{(1)}$}%{$\hat{K}_{\mathrm{OSPA}}^{(1)}$}%{associated (A1)}

\addplot [color=blue, dashed, line width=0.75pt,forget plot]
  table[]{\datapath/m120_fc6950MHz_bw0500MHz_K_CDF-3.tsv};
% \addlegendentry{$\hat{K}^{(2)}$}%{total (A2)}

\addplot [color=blue, line width=0.75pt]
  table[]{\datapath/m120_fc6950MHz_bw0500MHz_K_CDF-4.tsv};
\addlegendentry{$\vm{a}^{(2)}$}%{$\hat{K}_{\mathrm{OSPA}}^{(2)}$}%{associated (A2)}





\end{axis}
\end{tikzpicture}%


==> figures/m120_K_CDF/m120_fc6950MHz_bw0500MHz_K_CDF.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.971\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}},
xlabel={\#components},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={CDF},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1
]
\addplot [color=red, dashed, line width=1.0pt]
  table[]{\datapath/m120_fc6950MHz_bw0500MHz_K_CDF-1.tsv};
\addlegendentry{total (A1)}

\addplot [color=red, line width=1.5pt]
  table[]{\datapath/m120_fc6950MHz_bw0500MHz_K_CDF-2.tsv};
\addlegendentry{associated (A1)}

\addplot [color=blue, dashed, line width=1.0pt]
  table[]{\datapath/m120_fc6950MHz_bw0500MHz_K_CDF-3.tsv};
\addlegendentry{total (A2)}

\addplot [color=blue, line width=1.5pt]
  table[]{\datapath/m120_fc6950MHz_bw0500MHz_K_CDF-4.tsv};
\addlegendentry{associated (A2)}

\end{axis}
\end{tikzpicture}%

==> figures/m120_K_CDF/m120_fc6950MHz_bw1000MHz_K_CDF.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.971\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}},
xlabel={\#components},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={CDF},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1
]
\addplot [color=red, dashed, line width=1.0pt]
  table[]{\datapath/m120_fc6950MHz_bw1000MHz_K_CDF-1.tsv};
\addlegendentry{total (A1)}

\addplot [color=red, line width=1.5pt]
  table[]{\datapath/m120_fc6950MHz_bw1000MHz_K_CDF-2.tsv};
\addlegendentry{associated (A1)}

\addplot [color=blue, dashed, line width=1.0pt]
  table[]{\datapath/m120_fc6950MHz_bw1000MHz_K_CDF-3.tsv};
\addlegendentry{total (A2)}

\addplot [color=blue, line width=1.5pt]
  table[]{\datapath/m120_fc6950MHz_bw1000MHz_K_CDF-4.tsv};
\addlegendentry{associated (A2)}

\end{axis}
\end{tikzpicture}%

==> figures/m120_K_CDF/m120_fc6950MHz_bw2000MHz_K_CDF.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.971\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}},
xlabel={\#components},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={CDF},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1
]
\addplot [color=red, dashed, line width=1.0pt]
  table[]{\datapath/m120_fc6950MHz_bw2000MHz_K_CDF-1.tsv};
\addlegendentry{total (A1)}

\addplot [color=red, line width=1.5pt]
  table[]{\datapath/m120_fc6950MHz_bw2000MHz_K_CDF-2.tsv};
\addlegendentry{associated (A1)}

\addplot [color=blue, dashed, line width=1.0pt]
  table[]{\datapath/m120_fc6950MHz_bw2000MHz_K_CDF-3.tsv};
\addlegendentry{total (A2)}

\addplot [color=blue, line width=1.5pt]
  table[]{\datapath/m120_fc6950MHz_bw2000MHz_K_CDF-4.tsv};
\addlegendentry{associated (A2)}

\end{axis}
\end{tikzpicture}%

==> figures/m120_K_CDF/m120_fc6950MHz_bw3939MHz_K_CDF.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.9\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=35,
%xlabel style={font=\color{white!15!black}},
xlabel={number of estimated SMCs $\hat{K}^{(j)}$},
ymin=0,
ymax=1,
%ylabel style={font=\color{white!15!black}},
ylabel={CDF},
%axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(1.01,1)}, anchor=north west, legend cell align=left, align=left, draw=black,fill=white},
%extraAxisOptions,
% unit vector ratio=1 1 1
grid style=dotted,
major tick length=1mm,
clip mode=individual,
xlabel style = {yshift=1.5mm},
ylabel style = {yshift=-1mm},
]
\addplot [color=red, dashed, line width=0.75pt,forget plot]
  table[]{\datapath/m120_fc6950MHz_bw3939MHz_K_CDF-1.tsv};
% \addlegendentry{$\hat{K}^{(1)}$}%{total (A1)}

\addplot [color=red, line width=0.75pt]
  table[]{\datapath/m120_fc6950MHz_bw3939MHz_K_CDF-2.tsv};
\addlegendentry{$\vm{a}^{(1)}$}%{$\hat{K}_{\mathrm{OSPA}}^{(1)}$}%{associated (A1)}

\addplot [color=blue, dashed, line width=0.75pt,forget plot]
  table[]{\datapath/m120_fc6950MHz_bw3939MHz_K_CDF-3.tsv};
% \addlegendentry{$\hat{K}^{(2)}$}%{total (A2)}

\addplot [color=blue, line width=0.75pt]
  table[]{\datapath/m120_fc6950MHz_bw3939MHz_K_CDF-4.tsv};
\addlegendentry{$\vm{a}^{(2)}$}%{$\hat{K}_{\mathrm{OSPA}}^{(2)}$}%{associated (A2)}

\end{axis}
\end{tikzpicture}%


==> figures/m120_fc6950MHz_bw0500MHz_K_CDF/m120_fc6950MHz_bw0500MHz_K_CDF.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.971\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}},
xlabel={\#components},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={CDF},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1
]
\addplot [color=red, dashed, line width=1.0pt]
  table[]{\datapath/m120_fc6950MHz_bw0500MHz_K_CDF-1.tsv};
\addlegendentry{total (A1)}

\addplot [color=red, line width=1.5pt]
  table[]{\datapath/m120_fc6950MHz_bw0500MHz_K_CDF-2.tsv};
\addlegendentry{associated (A1)}

\addplot [color=blue, dashed, line width=1.0pt]
  table[]{\datapath/m120_fc6950MHz_bw0500MHz_K_CDF-3.tsv};
\addlegendentry{total (A2)}

\addplot [color=blue, line width=1.5pt]
  table[]{\datapath/m120_fc6950MHz_bw0500MHz_K_CDF-4.tsv};
\addlegendentry{associated (A2)}

\end{axis}
\end{tikzpicture}%

==> figures/m120_fc6950MHz_bw1000MHz_K_CDF/m120_fc6950MHz_bw1000MHz_K_CDF.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.971\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}},
xlabel={\#components},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={CDF},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1
]
\addplot [color=red, dashed, line width=1.0pt]
  table[]{\datapath/m120_fc6950MHz_bw1000MHz_K_CDF-1.tsv};
\addlegendentry{total (A1)}

\addplot [color=red, line width=1.5pt]
  table[]{\datapath/m120_fc6950MHz_bw1000MHz_K_CDF-2.tsv};
\addlegendentry{associated (A1)}

\addplot [color=blue, dashed, line width=1.0pt]
  table[]{\datapath/m120_fc6950MHz_bw1000MHz_K_CDF-3.tsv};
\addlegendentry{total (A2)}

\addplot [color=blue, line width=1.5pt]
  table[]{\datapath/m120_fc6950MHz_bw1000MHz_K_CDF-4.tsv};
\addlegendentry{associated (A2)}

\end{axis}
\end{tikzpicture}%

==> figures/m120_fc6950MHz_bw1000MHz_LOS_error_hist/m120_fc6950MHz_bw1000MHz_LOS_error_hist.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.971\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=-0.2,
xmax=0.4,
xlabel style={font=\color{white!15!black}},
xlabel={delay error in m (est-true)},
ymin=0,
ymax=300,
ylabel style={font=\color{white!15!black}},
ylabel={count},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1
]
\addplot[ybar interval, fill=red, fill opacity=0.5, draw=red, area legend] table[] {\datapath/m120_fc6950MHz_bw1000MHz_LOS_error_hist-1.tsv};
\addlegendentry{A1}

\addplot[ybar interval, fill=blue, fill opacity=0.5, draw=blue, area legend] table[] {\datapath/m120_fc6950MHz_bw1000MHz_LOS_error_hist-2.tsv};
\addlegendentry{A2}

\end{axis}
\end{tikzpicture}%

==> figures/m120_fc6950MHz_bw1000MHz_ampPL/m120_fc6950MHz_bw1000MHz_ampPL.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.951\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=-3,
xmax=3,
xlabel style={font=\color{white!15!black}},
xlabel={phi in rad},
ymin=-60,
ymax=40,
ylabel style={font=\color{white!15!black}},
ylabel={amp. in dB},
axis background/.style={fill=white},
title style={font=\bfseries},
title={with pathloss compensation},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1
]
\addplot [color=red, draw=none, mark=*, mark options={solid, red}]
  table[]{\datapath/m120_fc6950MHz_bw1000MHz_ampPL-1.tsv};
\addlegendentry{LOS amp. (A1)}

\addplot [color=blue, draw=none, mark=*, mark options={solid, blue}]
  table[]{\datapath/m120_fc6950MHz_bw1000MHz_ampPL-2.tsv};
\addlegendentry{LOS amp. (A2)}

\addplot [color=black, line width=2.0pt]
  table[]{\datapath/m120_fc6950MHz_bw1000MHz_ampPL-3.tsv};
\addlegendentry{g(\varphi)}

\end{axis}
\end{tikzpicture}%

==> figures/m120_fc6950MHz_bw2000MHz_K_CDF/m120_fc6950MHz_bw2000MHz_K_CDF.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.971\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}},
xlabel={\#components},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={CDF},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1
]
\addplot [color=red, dashed, line width=1.0pt]
  table[]{\datapath/m120_fc6950MHz_bw2000MHz_K_CDF-1.tsv};
\addlegendentry{total (A1)}

\addplot [color=red, line width=1.5pt]
  table[]{\datapath/m120_fc6950MHz_bw2000MHz_K_CDF-2.tsv};
\addlegendentry{associated (A1)}

\addplot [color=blue, dashed, line width=1.0pt]
  table[]{\datapath/m120_fc6950MHz_bw2000MHz_K_CDF-3.tsv};
\addlegendentry{total (A2)}

\addplot [color=blue, line width=1.5pt]
  table[]{\datapath/m120_fc6950MHz_bw2000MHz_K_CDF-4.tsv};
\addlegendentry{associated (A2)}

\end{axis}
\end{tikzpicture}%

==> figures/m120_fc6950MHz_bw3939MHz_K_CDF/m120_fc6950MHz_bw3939MHz_K_CDF.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.9\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=35,
%xlabel style={font=\color{white!15!black}},
xlabel={number of estimated SMCs $\hat{K}^{(j)}$},
ymin=0,
ymax=1,
%ylabel style={font=\color{white!15!black}},
ylabel={CDF},
%axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(1.01,1)}, anchor=north west, legend cell align=left, align=left, draw=black,fill=white},
%extraAxisOptions,
% unit vector ratio=1 1 1
grid style=dotted,
major tick length=1mm,
clip mode=individual,
xlabel style = {yshift=1.5mm},
ylabel style = {yshift=-1mm},
]
\addplot [color=red, dashed, line width=0.75pt,forget plot]
  table[]{\datapath/m120_fc6950MHz_bw3939MHz_K_CDF-1.tsv};
% \addlegendentry{$\hat{K}^{(1)}$}%{total (A1)}

\addplot [color=red, line width=0.75pt]
  table[]{\datapath/m120_fc6950MHz_bw3939MHz_K_CDF-2.tsv};
\addlegendentry{$\vm{a}^{(1)}$}%{$\hat{K}_{\mathrm{OSPA}}^{(1)}$}%{associated (A1)}

\addplot [color=blue, dashed, line width=0.75pt,forget plot]
  table[]{\datapath/m120_fc6950MHz_bw3939MHz_K_CDF-3.tsv};
% \addlegendentry{$\hat{K}^{(2)}$}%{total (A2)}

\addplot [color=blue, line width=0.75pt]
  table[]{\datapath/m120_fc6950MHz_bw3939MHz_K_CDF-4.tsv};
\addlegendentry{$\vm{a}^{(2)}$}%{$\hat{K}_{\mathrm{OSPA}}^{(2)}$}%{associated (A2)}

\end{axis}
\end{tikzpicture}%


==> figures/m120_fc6950MHz_bw3939MHz_ampPL_scatter/m120_fc6950MHz_bw3939MHz_ampPL.tex <==
% !TEX root = ../../2022_EuCAP_main.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\definecolor{mycolor1}{rgb}{0,0,1}%{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{1,0,0}%{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=-3,
xmax=3,
%xlabel style={font=\color{white!15!black}},
xlabel={$\varphi$ in rad},
ymin=-30,
ymax=20,
%ylabel style={font=\color{white!15!black}},
ylabel={$\hat{\alpha}_1^{(j)}$ in dB},
axis background/.style={fill=white},
%title style={font=\bfseries},
%title={with pathloss compensation},
xmajorgrids,
ymajorgrids,
major tick length=1mm,
grid style=dotted,
legend style={at={(0.5,0.01)},anchor=south,legend cell align=left,legend columns=3, align=left, draw=none,fill=none},
%extraAxisOptions,
% unit vector ratio=1 1 1
]
%\addplot[scatter, only marks, mark=*, color=mycolor1, mark options={}, scatter/use mapped color=mycolor1, visualization depends on={\thisrow{size} \as \perpointmarksize}, scatter/@pre marker code/.append style={/tikz/mark size=\perpointmarksize}] table[]{\datapath/m120_fc6950MHz_bw3939MHz_ampPL-1.tsv};
%\addlegendentry{${\alpha}^{(1)}$}%{LOS amp. (A1)}

\addplot[scatter, only marks, mark=*, color=mycolor1, mark options={}, scatter/use mapped color=mycolor1, visualization depends on={\thisrow{size} \as \perpointmarksize}, scatter/@pre marker code/.append style={/tikz/mark size=0.5*\perpointmarksize}] table[]{\datapath/m120_fc6950MHz_bw3939MHz_ampPL-1.tsv};
\addlegendentry{${\alpha}^{(1)}$}%{LOS amp. (A1)}

\addplot[scatter, only marks, mark=*, color=mycolor2, mark options={}, scatter/use mapped color=mycolor2, visualization depends on={\thisrow{size} \as \perpointmarksize}, scatter/@pre marker code/.append style={/tikz/mark size=\perpointmarksize}] table[]{\datapath/m120_fc6950MHz_bw3939MHz_ampPL-2.tsv};
\addlegendentry{${\alpha}^{(2)}$}%{LOS amp. (A2)}

\addplot[color=black, line width=1.25pt]
  table[]{\datapath/m120_fc6950MHz_bw3939MHz_ampPL-3.tsv};
\addlegendentry{$g(\varphi)$}

\end{axis}
\end{tikzpicture}%

